Documenting Data Production Processes: A Participatory Approach for Data Work

The opacity of machine learning data is a significant threat to ethical data work and intelligible systems. Previous research has addressed this issue by proposing standardized checklists to document datasets. This paper expands that field of inquiry by proposing a shift of perspective: from documenting datasets toward documenting data production. We draw on participatory design and collaborate with data workers at two companies located in Bulgaria and Argentina, where the collection and annotation of data for machine learning are outsourced. Our investigation comprises 2.5 years of research, including 33 semi-structured interviews, five co-design workshops, the development of prototypes, and several feedback instances with participants. We identify key challenges and requirements related to the integration of documentation practices in real-world data production scenarios. Our findings comprise important design considerations and highlight the value of designing data documentation based on the needs of data workers. We argue that a view of documentation as a boundary object, i.e., an object that can be used differently across organizations and teams but holds enough immutable content to maintain integrity, can be useful when designing documentation to retrieve heterogeneous, often distributed, contexts of data production.

==> Reserve/reserve.tex <==
\section{mila's reserve}

\subsection{Documentation \emph{for and by} Data Workers}

The co-design workshops that we conducted with both data worker groups constituted a turning point in this investigation.  Engaging in hands-on design sessions directly with data workers without the intermediation of their organizations gave us the possibility to explore their needs and desiderata beyond corporate priorities. Moreover, the workshops gave us and the three participant groups, i.e., data workers, managers, and clients, the possibility to learn about their relationship, communication, and cooperation.

Some of the ideas and requirements expressed by the participants were already present in the documentation prototypes previously developed by Action Data and Alamo respectively. However, there are several considerations\,---\,some subtle, some substantial\,---\,that should be taken into account if the aim is designing a data documentation framework based on the needs of data workers.  
In the following, we summarize and list some of these design considerations. %A prototype based on these considerations is part of the supplementary material.  

\subsubsection{Who are the documenters and who are the users of documentation?}

The first design consideration to take into account involves establishing the roles of each stakeholder in the documentation process. These roles can vary according to the company, the client, and the project.  There are, however, two patterns that can be derived from our findings:

\begin{itemize}
    \item Most of the information comes from the requesters and is documented by managers: The clients hold most of the relevant information and share it only with the BPO managers. The managers register that information in documents and act as gatekeepers, only granting access to the information according to the client's confidentiality-related requests.
    \item The data workers are expected to use the documentation: However, they receive only the bare minimum information that allows them to complete tasks according to client's instructions. Moreover, access is not always granted (as reported by Alamo's workers) and language translations can constitute a barrier (as discussed by Action Data's workers.)
\end{itemize}

Current documentation practices at Alamo and Action Data show a pattern of linear, top-down communication through documentation. Moreover, there is a discrepancy between how management thinks workers should use the documentation and the latter’s perceived usefulness vis-à-vis the time and effort required to maintain it. 

Such issues could be addressed by designers of documentation frameworks by clearly defining who is the user of documentation and designing with that user in mind. Breaking with patterns of top-down communication and gatekeeping by enabling feedback loops and promoting collaboration in the documentation process could be, in this sense, useful design considerations.


\subsubsection{What should be documented?}
The information that out participants considered relevant and should be included in the documentation of data production projects is:
\begin{enumerate}
    \item Who is the requester?: Information about the client, its products, and its relationship history with the data processing company. 
    \item What is the data going to be used for?: Description of the ML product that will be trained on the basis of the data produced by data workers. The connection between the tasks performed by data workers and its use for the resulting ML model should be highlighted.
    \item What kind of data are these?: Including a warning in case of sensitive data.
    \item Where do the data come from?: Description of data provenance and dataset's previous uses. Proof of compliance with local regulations in the case of personal data. 
    \item What should be done with the data?: Description of task including categories and classes for annotation and collection.
    \item How difficult is the task? How laborsome is this data?:  Include a difficulty rating for workers to quickly 
    \item What tools are used?: Include clear guidelines in terms of communication channels, software used to work on the data, and platforms where the data will be.
    \item Who is working on this project?: Include information about team composition.
    \item How much does this project pay to each data worker?: Include clear information about payment structure and rules.
    \item How has the project and its documentation evolved over time?: Include an updates history log, including date, time, and name of the person who documented each update.
    \item What have we learned from this project?: Include a post-mortem report to reflect upon edge cases, lessons learned, and possible mismatches between time, effort, and payment.
\end{enumerate}

\subsubsection{How should documentation be carried out?} Above-listed questions can vary and be adapted to different data-production scenarios. There are, however, three design considerations that should be taken into account regardless of the actual composition of the documentation template:
\begin{itemize}
    \item Communication and feedback: The participants prioritized documentation that is able to transport information about tasks and how to do conduct them.  They also expected documentation to be able to reflect workers feedback and communicate it back to the requesters. In this sense, task instructions could be co-created through iterations and communication enabled by documentation.
    \item Access and trust: The view of documentation as a communication medium between stakeholders, in this case, between requesters and outsourced data workers, surfaces tensions around how to access to sensitive information that requesters are reluctant to disclose. In this sense, the design of documentation frameworks should address this tension by enabling workers' access to information while provide enough security to requesters to trust the documentation process and disclose information.
    \item Input and output: the input of information in documentation (the act of documenting) and the use of that documentation (the act of retrieving information) require differentiated consideration and, often, some form of translation to ease mismatches. 
    In terms of information input, the participants expressed the need for the process to be simple and quick, preferably as a text-based, concise checklist or questionnaire that can be easily incorporated in day-to-day workflows. The output of documentation, however, was envisioned as detailed, well organized, and mostly visual. The mismatch between the desidarata expressed for the documentation input and output requires the integration of some sort of translation aid, in this case to turn a concise checklist into a compelling and visual document. 
    Translation can also be required in language terms, for instance, in the case of Action Data, where most of the information is documented in one language (English) but the documentation users need it in another (Arabic).
\end{itemize}


\section{workshop learnings}
%At the intersection of data collection, data annotation, and computer vision engineering, not every actor can influence decisions regarding what data to collect and how to label it \cite{miceli2020}.  In this constellation, requesters hold much of the decision-making power. However, they are not the most prone to documenting data production processes. Clients often regard some of the information that could or should be documented as confidential, especially if it involves details about the intended product or if some of the processes involved in producing the dataset are considered a strategic advantage.  Despite power imbalances (or maybe because of them), Alamo and Action Data appear to be more inclined towards documentation than their clients. 
%Knowledge + Accountability: Why are both important for transparency?
\subsection{alamo}

 %I added this because it is related to a question you raised in the recap: is the idea of wikis as sites for learning realistic? will workers really check other projects on wikis just for fun or out of curiosity or others? I thought this might be a question that others may have.
%for your reference:
%% B1: Yo quería sumar algo con respecto a ese punto porque me ha pasado varias veces que alguna persona venga y me diga: “Yo no sé qué otros proyectos hay en Arbusta”. Y luego vienes y le recuerdas que están las wikis. O sea, que como que por ahí no es algo que está muy por ahí presente, que saben que está y que lo van a buscar. Quizás falta eso, un poco de difusión, de saber que está, que existe algo donde están todos los proyectos, que cualquiera lo puede ver. Y que, si les interesa, ese es el lugar donde lo van a tener. No sé si toda la información, pero algunos puntos van a sacar. (DIA2 ACT4+5Intro - Transkript - TR217626, Pos. 37)
%% B3: Bueno, yo creo que de pronto lo que nos falta es que, por ejemplo, yo en este momento tengo acceso a la wiki de machine, pero de pronto no tenemos como esa visual de, “bueno, me voy a meter a ver el de data” o, como decía Renzo ahorita, “a ver el de testing”, como decía Renzo ahorita. No tengo como acceso a esos documentos, o al menos no tan a la mano como de, “ve, en este momento me surgió mirarlo y lo voy a ver”. Como que no está tan a la mano. Tengo el de machine sí, ahí yo lo busco y está, porque es el del proyecto en el que estoy, pero muchos de los chicos de pronto no saben en realidad qué se hace en otros proyectos, y ahí creo que hace falta eso. (DIA2 ACT4+5Intro - Transkript - TR217626, Pos. 39)
%% B3: Yo creo… Por ese lado es más como para que los chicos puedan ver la documentación. Por ese lado he visto que, si desde que se empieza a capacitar, desde que se empieza el onboarding, se les recalca que es muy importante que estén pendientes de la documentación, que estén como… que la tengan todo el tiempo abierta, funciona. Y estén de pronto más atentos, más pendientes y no preguntan tanto, porque de pronto antes teníamos como otro proceso que era que iban primero al QA, que son como los que tenían los conocimientos, entonces siempre acudían al QA que les iba a estar respondiendo. Lo que hace que de pronto se quita esa tendencia del QA y se les recalca desde el inicio que estén pendientes de la documentación, que la mantengan abierta. Ellos, los que la han cogido ya en este último tiempo, están pendientes. Tú te metes en la documentación y la documentación está abierta. Lo ven, y si alguno tiene una duda como un criterio, pregunta y los otros chicos le dicen: Mira, esa parte está en tal y tal parte de la documentación. Entonces, digo que, por ese lado, estaría chévere empezar con todos y que tengan ese criterio.  (DIA2 ACT4+5Intro - Transkript - TR217626, Pos. 59) 

\subsection{action data}
%connected to design ideas - information type, but not sure if this fits here: In the round for open questions at the end of this session, a worker asked why animals were not required for annotation despite their occurrence in videos. A client explained that there might be several reasons: it could be that they did not ask for annotation of animals due to limited budgets, or they were not aware that animals were spotted in the videos, or the low frequency of occurrence of animals in the videos means that they are not very useful for the development of machine learning models. A manager then proposed that this might be the moments of documentation - when certain things were not required for annotation but still appeared in the videos. (DAY2 Act1+2Intro - Transkript - TR217631, Pos. 43-51.) 

%In one of the breakout groups, the participants were planned to be several data workers, one manager from Ranua and one from Action Data, who did not participate in the group activity because she had left the workshop earlier. The breakout group had one interpreter and one secondary facilitator who spoke Arabic. While the result was a prototype for documentation, it resulted mostly from the design ideas the facilitator came up with together with the manager from Ranua. One possibility is due to the translating back and forth between the two languages or because the data workers wanted to allow him to speak first.   
%Mohamed tried to include the others but they did not speak up. Why? Were they afraid to talk in front of a manager who might know better? Was it the language barrier, since Mohamed speaks fluent English and they don't? Mohamed himself however was very engaged. Also this is something about the online setting but, no one had their webcam on except Julian and I always feel like if the webcam is turned off, dialogue is a bit harder...

\section{Sonja's Notes}

%Giving equal voice to different types of knowledge and at the same time respecting the different views – and worldviews – is not easy. In his theory about ‘model power’, Bråten (1973) argues that our worldviews and understandings are crucial for knowledge acquisition and decision-making. Our ways of understanding, i.e. our ‘models’ of the world, constitute the basis for how we can utilise information. Information needs to be organised, sifted and processed, and it is the processing of information into a meaningful context, just as much as the information pieces themselves, that gives us knowledge. Bråten therefore suggests that the model into which the information is interpreted or contextualised provides the originator of a model with symbolic power. Adopting somebody else’s model will give the originator ‘model monopoly’ (ibid.). The model defines the universe of discourse and the scope of the decisionmaking. New information will only strengthen the model originators’ position as they have a richer image of the universe of discourse than the model-weak party, who may not be able to utilise the new information to the same extent. When one model defines the discussion, the relationship between the ‘model rich’ and the ‘model weak’ is asymmetrical and continues to be so.
%Model monopoly can be challenged by addressing the model power mechanisms. Changing the premises for model monopoly involves expanding the universe of discourse to also include areas outside the original model. Participatory Design methods do this by insisting on taking use practices as a basis for design, rather than any formal representation of use activities or technical matters. Inviting more stakeholders into the design process expands the universe of discourse, treating all worldviews as equally important – hence there is no one model of the world.


%Reflecting on the work as a part of a mutual learning process can make procedures, skills, assumptions that are involved in the work come to the foreground subject them to evaluation and change, leading to a new understanding and opportunities for change. Participatory Design methods hence emphasise using both concrete experience and abstract descriptions of knowledge: the concrete experiences are necessary for concrete discussions about future (work) activities and for judging the relevance of abstract descriptions, and the abstract descriptions are necessary for discussing the larger picture and how a new technical solution will affect the organisation as a whole"\cite[p.135]{routledge_methods}.

%Co-realisation is an important aspect of Participatory Design projects because it is difficult to imagine technical possibilities for users. Visualising possible solutions comes into play here, for example via prototyping. A prototype as a tangible artefact "makes it easier to imagine the consequences of a design suggestion than would and abstract description". The prototype can be evaluated by users through their professional competence. 

%Co-realization is about involving participants in designing. Participatory design emphasizes different ways of visualising possible solutions by using tangible artefacts, such as prototypes. Imagining the consequences of a design suggestion is easier, if a tangible artefact is available for evaluation, instead of an abstract description\citet{routledge_methods}. To facilitate \emph{co-realization} through the proposed workshop activities, we used different symbols. For instance, for the activity "Re-imagining documentation" we used both visual and text-based input to ask participants to gather in groups to design a documentation framework for a given project. The symbols were used to give some suggestions, however it was made clear by the facilitators that other options were very welcome. 

%briefly explain what participatory design is
%which co-design form / school did we apply in this paper?
%why participatory design? How does this method align with our research goals?
%How did we apply it? --> I think the next subsections (especially Sample) should give you a decent idea of what we will describe in this paper 
%OPTIONAL: some challenges to take into account in co-design and that appeared in our case? E.g. power asymmetries during the workshops

%challenges: do we want to include this?
%When working with participants, there are considerations to take into account. Robertson and Wagner mention some core considerations: how to deal with sensitive topics, how users can be made to feel confident and secure, how risks of embarrassment and unpleasant surprises can be avoided, and what steps are necessary to protect the participants' privacy\cite[p.74]{routledge_ethics}.

\subsection{Participatory Design}

%cscw read how other papers describe it

This section gives a short overview of Participatory design (PD) principles and the way we embedded them into our research. The PD methodology we are following emerged in Scandinavia in the 1960s and is the "process of investigating, understanding, reflecting upon, establishing, developing and supporting mutual learning between multiple participants in collective 'reflection in action'."\cite{routledge_introduction}. Co-design is often used as an umbrella term for various participatory design approaches, and we will use both terms as synonyms throughout this paper\cite{costanza-chock2020}. Using participatory design expresses the ethical stance of respecting people's expertise and right to represent their own activities to others, instead of having others do it for them. To us, it was very important to allow the data workers to represent and describe their work and expert knowledge to the other stakeholders present at the workshops.

A central motivation in PD is the "interest in empowering users"\cite{asaro_2014_pd}, as they are seen as active participants in changing the world around them\cite{routledge_ethics}. We wanted to enable the data workers to describe their current work practices and (possible) problems arising with current data documentation practices to find possible improvements.

Bratteteig et al. argue that a technical solution is "developed by someone for someone and [...] implements a particular worldview"\cite{routledge_methods} which is why all stakeholders should be invited to discuss solutions. !!Add here that we invited all stakeholders and explain why!! This view leads to three core perspectives for participatory design: \emph{having a say, mutual learning} and \emph{co-realization}\cite{routledge_methods}.

While conducting this investigation, we were intentional about listening to what the different actors involved in data production (the data workers, their managers, and the clients) had to say about dataset documentation, in order to develop a framework that would adapt to their needs and desiderata. As our research project evolved, we especially focused on the experiences of the data workers because we realized they were the ones that usually did not \emph{have a say} in how workflows and processes are designed in ML supply chains. We will discuss this shift of perspective in Sections 4.

Mutual learning enables all participants to know enough about the whole area to understand each other's expertise and develop mutual respect. This is the basis for a discussion on equal terms\cite{routledge_methods}.To foster \emph{mutual learning}, we designed workshop sessions involving data workers and their managers. In order to enable the participants to present their work practices to the others, we prepared activities that allowed participants to tell about important aspects of their work. This included information such as communication patterns and describing the processes and tasks involved in the production of ML datasets. Moreover, and since there is normally no direct contact between the data workers and the requesters, having one of Action Data's client joining for a three-hour workshop session offered a great opportunity for the data workers, the managers, and the requester to enter a dialogue and learn about each other's goals and concerns. An example of this is one of the activities carried out at that workshop session which included a role play in which the participants were asked to assume the role of another group of stakeholders. 
All stakeholder groups had the opportunity to assume the role of another stakeholder and assume their view, but also to hear about whether their assumptions about what information is needed aligned with reality.

Fostering mutual learning was fundamental to us throughout the design process. As we will describe in Findings, not only did we learn from the participants and their experiences but also put effort in providing feedback and engaging in conversations with the participants as we analyzed the collected data. In this sense, the participants expressed on several occasions having learned or realized things from the interactions created during the interviews and at the workshops. 

%To promote mutual learning, Bratteteig et al. mention three important aspects: identifying and defining problems, envisioning by developing ideas about possible technological designs as parts of future use practices, and concretizing ideas through sketching or prototyping. Participatory Design methods are explorative and aim for the inclusion of decisions about which problems are to be solved\cite{routledge_methods}. 

%We used different symbols to concretize ideas. For instance, for the activity "Re-imagining documentation" we used both visual and text-based input to ask participants to gather in groups to design a documentation framework for a given project. The symbols were used to give some suggestions, however it was made clear by the facilitators that other options were very welcome. 
%these two paragraphs are kinda together. discuss which to use.

\subsection{Thematic Analysis}

%Notes from Sonja to go over this and see what should be included
%Gareth and David again worked independently and collaboratively in the early stages of theme construction, meeting regularly to discuss candidate themes. Their meetings took the form of a kind of “theme off”: each presented their candidate themes, including preliminary theme names and definitions (discussed soon); they then “tussled” with each theme, and the collection of themes, to identify the most meaningful potential themes, the ones that collectively told the best story of the data. Thematic mapping – a process of visually exploring potential themes and subthemes, and connections between them (Braun and Clarke 2006) – was useful. Figure 1 maps the six candidate themes produced through this process, with all being relevant to the research question. Three of the initial themes Gareth and David constructed independently were similar enough to collapse into the single “bodies about more than roles and functions” theme – Gareth had identified a theme called “multiple embodiments”; David had two called “demanding embodiment” and “knowledge about bodies.” Their process demonstrates a way of working together, analytically, outside a consensus-building model.
%The phases of revising and defining themes are particularly important, precisely because candidate themes are effectively prototypes. Sometimes they do not work! It can be difficult to “let go” of our early ideas, but holding too tightly to a candidate theme can potentially result in analytic “thinness” or conceptual overlap. The story being told about the data risks being diminished in richness, or conceptually confused, by inclusion of weak or overlapping themes. Having clear definitions of each theme – a paragraph delineating the theme’s boundaries and central organizing concept (for examples, see Terry et al. 2017) – helps clarify the essence and scope of each theme. Indeed, it was such descriptions of Gareth and David’s three candidate themes that highlighted their similarity and led to combination as a single theme (note that typically, not every facet survives this review process!).

%In their book "Successful Qualitative Research" Braun and Clarke write this about reflexivity: (This is the book I wanted Evelyn to buy, I hope it will arrive in early January so that I can go through it before submission)
%"Reflexivity – critical reflection on the research process and on one’s own role as researcher (Finlay, 2002a, 2002b), including our various insider and outsider positions (Gallais, 2008). We have insider status when we share some group identity with our participants – for example, a male researcher researching men would be an insider; we have outsider status when we do not share some group identity with our participants – for example, a white man researching Asian men would be an outsider. For any research, we are likely to have multiple insider and outsider positions."

\section{Ling's notes}
\subsection{For revision}
Find relevant quotes in: https://docs.google.com/document/d/17180KH1q5RK7bmv3RGJjGTKNBIUDIx8YaWreJqCncGg/edit?usp=sharing
This document includes quotes for: 1) Difference across sites in workshop data (general); 2)
 Why workers want to see those elements documented & Difference across sites in Section 4.3; 3) Trust (R2's comment). Important quotes are marked in red.

\subsection{Previous notes}
%Jo and Gebru \cite{jo2020} adapt practices from archives and libraries to ML settings and advocate for adopting a supervision system of multiple layers and actors to promote ethical practices in data collection and hold those who violate code of ethics accountable. Similar to Jo and Gebru's approach \cite{jo2020}, Famularo et al\cite{famularo2021} draw on the parallel between GLAMs (galleries, libraries, archives, and museums) and ML. Introducing the concept of stewardship, they broaden the scope of involved stakeholders and the potential contexts to be investigated beyond original production and intended use of datasets. While most foregoing studies are oriented towards impacting data and documentation practices in the future, Scheuerman and colleagues \cite{scheuerman2021} reorient the focus on existing data and documentation practices, with special attention to the values that are prioritized and guide current dataset development and practices. They advocate for attaching datasets to a fixed doi and storage location that enable persistent reference to the data and version control of the data. A data maintenance plan is also recommended to not only guarantee the accessibility to the data but also raise the transparency of changes and updates made on the data.

%When difficulties arise in the communications and practices on a common object that has both shared and local meaning across multiple contexts and communities, a common solution is standardization or formalization \cite{bowker1999}. However, standards and routine practices in one group might result in confusion in another group \cite{Gasser1986}. Prescribed standards and formalized artifacts also often fail to accommodate local specificities and constraints. In particular, Suchman \cite{suchman2002} advocates for "artful integration" both among devices and between the design and use of devices over decontextualized and homogeneous artifacts. When such artful integration involves continuous and relatively stable relationships among different communities and shared objects jointly produced by them, "then boundary objects arise"\cite{Bowker1999}.
%We argue that the concept of boundary object can provide a potential solution to the difficulties arising from coordinating and collaborating across communities and contexts. 

%A library is an example of boundary object. In a library, collections are ordered in an indexed and standardized manner that allows people to use for their own purposes - people can access and borrow books via the library management system without the need to further negotiate their different purposes.

%a prevailing assumption in the research on collaborative work in document construction is that collaborators are willing to share information with others openly and as much as possible and work under a common goal, which Cohen and colleagues refer to as cooperative collaboration \cite{cohen2000}, but this is only part of the story.

%Boundary objects are flexible enough to adapt to the requirements of different organizations and communities but, at the same time, maintain certain level of integrity and common identity\cite{star1989, bowker1999}.  
%Another example can be various maps of same city made by geographers, citizens and biologists. They have the same geographical boundary but vary in contents and uses, depending on different groups that create them. This way, boundary objects can foster and facilitate coordination and collaboration on common tasks or topics despite the multiplicity and heterogeneity of involved actors and communities and the varying goals，interests and needs they have. 

%The notion of boundary object has been used in documentation and exploration of interdisciplinary and multicultural research projects\cite{light2009}, in medical and health records \cite{bossen2014}, and in everyday situation such as a wedding planning guide \cite{mckenzie2009}. Specifically within CSCW, Bossen et al \cite{bossen2012} conceive the coordination mechanisms that facilitate communication and collaboration among different actors in the hospital as boundary object and coin the term \emph{boundary-object trimming} to explore the interaction and work in medical secretaries' care for records that otherwise remain invisible. Lutters and Ackerman \cite{lutters2002} investigate the use of boundary objects by service engineers in an aircraft technical support center to achieve safety. 
%This notion is also used to study organizational memory \cite{ackerman1998} and common information space \cite{bannon1997, schmidt2008}. Previous work has also pointed to its limitation in capturing short-lived, situated and fluid arrangements \cite{rolland2006, lee2005}. Lee\cite{lee2005, lee2007} further coins the term \emph{boundary-negotiating artifacts} to explore non-standardized, fluid and informal objects that not only travel across but also destabilize and push boundaries. 

%- Bossen, C., Jensen, L.G. & Udsen, F.W. Boundary-Object Trimming: On the Invisibility of Medical Secretaries’ Care of Records in Healthcare Infrastructures. Comput Supported Coop Work 23, 75–110 (2014). https://doi.org/10.1007/s10606-013-9195-5 
%As boundary objects themselves are diverse, four main types of boundary objects are identified, namely, repositories, ideal type, coincident boundaries and standardized forms \cite{star1989}. Repositories refer to objects ordered in an indexed and standardized manner that allow different actors and communities to use for their own purposes. Libraries can be an example of repository, as people can borrow books from them without the need to negotiate their different purposes. Ideal type refers to an object that is an abstraction of the thing described across domains but does not address its details. Coincident boundary refers to an object with the same boundary but different contents for different groups. For instance, the maps of the same city created by geographers, citizens and biologists are different. Standardized form is the object that enable different groups to communicate in a standardized and common way. For example, registration forms for all participants in an event can keep record of standardized information and reduce local uncertainties.
%notes for discussion part:
%%Huvila, I. (2011). The politics of boundary objects: hegemonic interventions and the making of a document. JASIST, 62(12), 2528–2539.
%%some connections: boundary object as an evolving project; boundary object as artifact(s) (the material aspects); boundary object as an interface/ a common communicative space (a consensus among all involved communities is not necessary; it can be a point of reference and also a space for discussion and negotiation)


Analyzing how choices are opened and closed and who participates in decisionmaking
as an element of PD practice leads to a more precise understanding of the
practical limitations of participation in design, some of which point to power issues.
We consider the notion of ‘power to’ (Pitkin 1973) a useful concept for PD. ‘Power to’
means agency: the capacity to shape action, which partly depends on access to
organizational resources, partly on ‘power/ knowledge’ in the Foucault sense (e.g.
Foucault 1972). Hence, the second part of our analysis looks into what shapes the
possibilities for participation, looking at: the institutional framing of the projects; the
sources of power and influence different project participants were able to mobilize; the
linkages between the decisions that influenced the dynamics of decision-making in the
projects. The decision-making framework we will introduce is intended as a tool for
‘reflection-on-action’ after a project has been completed; but also as a tool to reflect on
power and decision making when taking moves as designers in the design process.

PD is a special kind of cooperative design process, with a focus on enabling different
stakeholders with different perspectives and competencies to cooperate. The focus of
CSCW is on understanding collaborative work practices and the details of the working together more generally (see e.g. Schmidt 2014), including design
practices. In this sense CSCW and PD are addressing the same phenomenon,
assuming somewhat different perspectives.

\section{Information on papers about PD}

\subsection{Culture in Action}

We contribute to HCI scholarship by further
discussing 1) how to analyze capacities’ design potential, and
2) the methodological particularities for collecting them.

\paragraph{What theories did they follow?}

- assets-based design: design starts from deep understanding of people's assets instead of needs and deficits
- cultural sociology and shifting emphasis from assets to capacities: Swidler's theory of culture-in-action as analytical lens for unpacking complex relationship between capacities, goals, structural limitations

\paragraph{What is their contribution?}

We contribute to HCI scholarship by further
discussing 1) how to analyze capacities’ design potential, and
2) the methodological particularities for collecting them.

\paragraph{What did they write in their methods section?}

"We wanted to provide a trusting third space" and then cite:
Homi Bhabha. 2004. The location of culture. 1994.
London and New York: Routledge (2004), 5–6.

Michael J Muller. 2009. Participatory design: the third
space in HCI. In Human-computer interaction. CRC
press, 181–202.

Jesper Simonsen and Toni Robertson. 2012. Routledge
international handbook of participatory design.
Routledge.

Lindsay Vecchio, Karamjeet K Dhillon, and Jasmine B
Ulmer. 2017. Visual methodologies for research with
refugee youth. Intercultural Education 28, 2 (2017),
131–142.

Tscheligi et al. (1995), in a panel on prototyping, considered that the “products” of
prototyping include not only artifacts, but also understandings, communications, and 
Participatory Design - 6 - Michael Muller
relationships – a theme that was echoed in a more recent panel on modeling (Kaindl et
al., 2001). 

Each
world has its own knowledges and practices; each world has well-defined boundaries.
Movement from one world to the other is known to be difficult. We can see this
difficulty manifested in our elaborate methods for requirements analysis, design, and
evaluation – and in the frequent failures to achieve products and services that meet users’
needs and/or are successful in the marketplace.
Traditional scientific practice in HCI has focused on instruments and interventions
that can aid in transferring information between the users’ world and the software world.
Most of the traditional methods are relatively one-directional – e.g., we analyze the
requirements from the users; we deliver a system to the users; we collect usability data
from the users. While there are many specific practices for performing these operations,
relatively few of them involve two-way discussions, and fewer still afford opportunities
for the software professionals to be surprised – i.e., to learn something that we didn’t
know we needed to know.
The PD tradition has, from the outset, emphasized mutuality and reciprocity – often
in a hybrid space that enabled new relationships and understandings. Bødker, Knudsen,
Kyng, Ehn, and Madsen (1988) made specific references to “the mutual validation of
diverse perspectives.” Floyd (1987) analyzed software practices into two paradigms,
which she termed product-oriented (focused on the computer artifact as an end in itself)
and process-oriented (focused on the human work process, with the computer artifact as
means to a human goal). I

%I rewatched my video. Here is my summary of what happened. I know you told me to put things here and you would accept the changes. But I definitely cannot put this into nice words. So what happened in my group with this activity was: I explained what the task is, reading out the example question. Tess told me she did not understand why I ask her the question of what the client needs and told me the client is not back yet. She said "Sonja, I don't know who you are directing this question to, but just letting you know that the clients are obviously not back yet." I proceeded to tell her that we are doing a roleplay and it's intentional that she is NOT the client. She muted herself, made some gestures and talked to someone else. I told her that I cannot hear her. She said again "All your questions are directed towards the client and they're not back yet." I said it was not a mistake, it was on purpose and that the clients have to do their own roleplay. "We are trying to put ourselves in the shoes of another stakeholder", then Adriana came in to tell me something. I explained the task again, Adriana was still there. Then Tess said interrupted me and said: "I didn't understand the task because I was not 100% listening in the whole conversation. Now I did it." So she finally understood the task. She told me to make the screen bigger (Me being confused because I thought it was big enough). Again, I read out the task. She said I am not an engineer, I don't know but "from my perspective" and proceeded to tell me stuff. She then asked Yalda if she has any ideas and then started doing something else (she even got up and left her seat, leaving her mic on...). While Yalda talked she also talked to some other guy and took off her headphones, so she definitely did not hear anything Yalda said. In the last 30 seconds Mohamed started speaking up. Yalda too, and they told each other you go ahead. It was also a bit my fault because I let Tess and Yalda both talk so long. It felt like Mohamed wanted to let the other two finish first. I negotiated that everyone presents the question they thought of. However, Yalda and Tess left before our presentation. This also means that Tess and Yalda did not hear about our stakeholder's views on their role. To be honest, internally I felt really annoyed and disrespected by Tess, because she made me repeat the task three times and tried to explain to me that I had made a mistake when it was her... of course I didn't let that show.

For terms such as tools and toolkit, the definitions by Sanders and Binder will be used. They define tools as "the material components that are used in PD activities", toolkits as "a collection of tools that are used in combination to serve a specific purpose". A technique describes how the tools and toolkits are put to use, such as being "sorted, categorized, prioritized, used to make a collage, tell a story and/or used to spark conversations"\cite[p.196]{brandt_framework}. A method is "a combination of tools, toolkits, techniques [...] that are strategically put together to address defined goals within the research plan"\cite[p.196]{brand_framework}. They define approach as describing "the overall mindset with which the research plan is to be conducted", which can be, for example, participatory.
 p.85:  These include participatory design (PD), user-led innovation,
user-centered design (UCD), human-centered design (HCD), inclusive
design, and codesign, among a growing list of terms and acronyms
p.88: An extensive community of practitioners and scholars also clusters
around the term codesign, often used as an umbrella that includes various approaches to PD and HCD. This approach is reflected in the journal CoDesign, in annual codesign conferences, and in the appearance of
the concept across multiple fields.page 11: Codesign, a closely allied approach, can be traced to Scandinavian efforts in the 1960s and 1970s to include both workers and managers in sociotechnical systems design. Both PAR and codesign consider
communities to be co-researchers and co-designers, rather than solely
research subjects or test users.

==> Reserve/reserve2.tex <==
\section{Findings}

\subsection{Lessons from the Interviews}
\label{sec:FindInt}

\subsubsection{Alamo's Documentation Practices} 
Through events and courses offered in poor areas of Buenos Aires, Alamo targets young workers from impoverished neighbourhoods and favors those without previous experience in the tech field. At fieldwork in 2019, one of the observations that stood out was the company's stated commitment to foster its workers' professional growth. In contrast with this mission, Alamo's documentation practices seemed, in 2019, almost completely oriented towards surveilling workers and measuring their performance. Noah, one of the data workers that we interviewed in 2019 described the documentation process as follows: 

\begin{displayquote}
For instance, for this project, we have three metrics for individual performance and now we're about to add one more. Mostly, we quantify and document errors or rollbacks reported by the requester.
\end{displayquote}

Nancy, who was one of Alamo's project managers in 2019, explained what was done with the documented performance metrics:

\begin{displayquote}
Within the company's structure, QA [the quality assurance department] then takes those metrics and puts together something like a “scores board” that shows everyone's performance and that is visible for the whole company.
\end{displayquote}

After our first fieldwork period and once we had analyzed the collected data, we provided Alamo with a report summarizing our observations. \textcolor{red}{We have discussed those observations and their implications at length in previous work (REFERENCES ANONYMIZED)} We found that there was a contradiction between the company's mission of fostering worker growth and its emphasis in quantifying individual performances, and suggested reorienting the purpose of documentation to include information that could help workers understand the background and purpose of their work. After presenting our observations, we engaged in a conversation with Alamo's co-founder Priscilla who, as shown by the next interview excerpt, agreed with our suggestions and expressed her desire of establishing documentation practices based on the needs of data workers:

\begin{displayquote}
\textcolor{red}{In my opinion, this is what we need to do.  Listen more to their needs and ask them what they need to perform better and do their work better. And we must generate and provide the information they need.  We need to make time for that.}
\end{displayquote}

In September 2020, we resumed contact with Alamo's management and invited the company to participate in our investigation on data production documentation, starting with a series of follow-up interviews. By then, the company was already in process of re-structuring its documentation practices. Nati, one of Alamo's former QA analysts, had just been promoted to “continuous improvement analyst” and put in charge of bringing together the company's quality standards and its goals in terms of promoting workers' professional growth. Nati's main task was re-designing Alamo's documentation practices. She described this process as follows:

\begin{displayquote}
During the past year, we made an effort to ask everyone “what would you like to see reflected in documentation? what do you need.” After that, we started dropping old practices that didn't make sense anymore, we threw them away, and started anew. We learned a lot, about empathy too, you know? This work is very much about empathy [...] because we assign workers in each team according to their competences, their skills, and they need to know what projects are about to actually make the most out of those skills. 
\end{displayquote}

What came out of the process led by Nati was a series of documentation practices strongly oriented towards \emph{knowledge preservation}, i.e., the documentation of workflows, tools, specific details about the conduction of projects, best practices, and lessons learned. In Nati's words, documentation was envisioned as an educational resource for Alamo's workers and its aim was mitigating information loss due to fast worker turn around. A special team led by Nati was put in charge of developing and implementing this vision. With the documentation guidelines and templates designed by them, each team leader would document the projects carried out by their data workers. Moreover, following one of our suggestions, the company saw value in documenting contextual information about the ML products that are trained or validated using data produced at Alamo. Management then started to seek clients' involvement in documentation practices. The first step was sharing the project documentation with the project's requester and asking for feedback. These collaborative practices progressed to the point that some clients became co-producers and users of the documentation produced by Alamo, as Pablo, leader of one of Alamo's data labeling teams described:

\begin{displayquote}
I mean, it depends on the client. Luckily this requester is very committed and is always looking at our documentation, providing feedback, checking if the information is up to date. Sometimes they just jump in and add information, they collaborates on the best practices manual. It's also good for them to see if their information is updated too, not just for us, but for the requester's own team, because they share these documents within the requester's company.
\end{displayquote}

%We had the chance to interview one of those requesters, namely an engineer working at a Barcelona-based company developing computer vision technologies. His perception of these collaborative documentation practices was overall positive, especially in regard to the communication of task instructions and the possibility of making sure that workers understood instructions as intended by his engineering team:

%\begin{displayquote}
%This has been good for both parties and we have discussed this with my team. Good documentation helps a lot to know where flows can be improved, what things can become a problem, and so on.
%\end{displayquote}

While this arrangement was beneficial for the clients, Alamo was providing the infrastructure and most of the workforce that made documentation possible. Alamo's workers started to feel the burden, as team lead Pablo described: 

\begin{displayquote}
We definitely noticed the change: from not documenting at all to documenting everything. It also depends on the project, for instance, our main client [a large regional e-commerce corporation] brought many more requirements for us to implement in our documentation in terms of what they wanted to see reflected. There are new documents and new guidelines all the time. 
\end{displayquote}

We followed up with continuous improvement analyst Nati in December 2020 as she continued to review and revise documentation practices within Alamo. By then, Alamo's documentation revolved around two templates that were to be implemented in each project conducted by the company: one known as the \textit{Kick-Off Document} and the other called the \textit{Wiki}.  The Kick-Off Document was a slide deck where basic information about Alamo's relationship with the requester was registered, i.e., the service to be provided, deadlines, contact information, and responsibilities. Instead, the Wiki was conceived as a collaborative document that enabled the conduction of projects (see Fig. \ref{fig:wiki}). Each Wiki comprised information, collected in many cases in direct collaboration with the requester, about processes, tools, and best practices concerning each specific project. Nati's main concern back then was reducing the time and effort that were flowing into documentation and, at the same time, finding efficient ways of keeping documentation updated. 
%She had audited some of the metadata that had been generated since the implementation of these new documentation templates, and had found that much information was redundant or hard to find.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.40]{alamo_wiki.pdf}
    \caption{The wiki-based documentation prototype created by Alamo to brief and train workers.}
    \label{fig:wiki}
\end{figure}

After these interviews with Nati, Pablo, and some other data workers, we got back to Alamo's management with feedback. Among other things, we highlighted the need to reduce the amount of work put on Alamo's team in terms of producing and maintaining documentation, and to distribute responsibilities more equitably.  The idea of producing exhaustive metadata for each project was commendable but the price of such an effort was being paid by the data workers.  Moreover, we found that the original idea of the Wikis, namely, that of preserving the knowledge generated in each project and offering more information about the machine learning supply chain to foster workers professional growth, had shifted towards a constant consideration of what clients might want to see reflected in documentation, as Sole, leader of another one of Alamo's data labeling teams, described:

\begin{displayquote}
We need to know what we want to document first.  Who we are documenting for.  That's a challenge at the moment. Because right now I ask myself: who am I doing this for? What for? […] Right now, we're focusing on the clients: what is the client asking for? Because I may want many things but, what is the client interested in? What is the client expecting from us as service providers?
\end{displayquote}

In view of these challenges, we proposed the idea of conducting a series of co-design workshops with Alamo's data workers and managers with the purpose of moving the focus away from “what clients want” and re-imagining documentation based on the needs of workers. In June 2021, we started conversations with Alamo.  %Points of discussion included participants' compensation and attendance, i.e. how many and which workers would Alamo allow to participate in the workshops. 
We agreed to use the Wiki as the prototype we would discuss and re-imagine at the workshops. After several months of negotiation, the workshops finally took place in October 2021 (see Section \ref{sec:workshops-alamo}).

\subsubsection{Action Data's Documentation Practices}

Our first approach to Action Data was in July 2019 as we spent several weeks at the company's office in Sofia, Bulgaria, conducting observations and interviews with data workers and management (REFERENCE ANONYMIZED). Back then, the company was handling projects with a pool of around 60 free-lance data workers, mostly immigrants from the Middle East living in Sofia. Projects and workers fluctuated frequently and communication seemed to adapt to the needs of each project. %The company's management communicated with clients in English and with data workers either in English or Bulgarian. Often, however, language translation was needed, depending on which data workers were assigned to work on each project. In such cases, one worker with knowledge of English would translate the task instructions, communicate updates from the requester, and mediate in cases where other workers needed clarification. 

%Sarah is one of the data worker that in 2019 was serving as as a translator for her non-English speaking colleagues. 
%She is a single mother and lives with her two young children in Bulgaria under refugee status after escaping Afghanistan by road with a toddler and being pregnant. Her second son was born on the road and became severely ill. He needs permanent medical attention. 
%She described her dual role as a data worker and mediator as follows: 

%\begin{displayquote}
%B: I’m a translator for four people here from Afghanistan. The other ones are calling me, “Sarah, I’m having a problem in this area. What to do?” Because every time I’m coming with them when Eva giving them training, I am seeing the work, I know work of everyone. Not only the, what she is doing, what the other one is doing because they are translating everyday I’m coming and I’m seeing their work. And first I’m learning and then I’m telling to them. 

%I: Okay and then what happens if they have questions or problems? 

%B: She [an Afghan colleague of Sarah] is calling me and showing me her screen that we have problem here like when she forget the names in English. And she's asking what was this and sometimes she's showing that why it’s not selecting. I don’t know then I’m saying, “you have to refresh or you have to sign out and come back sign in” like these things. 

%\end{displayquote}

In 2019, %most of the worker training was done in-person and orally in the company's office. %After the training was completed, workers would sign an acknowledgement form documenting that they have received the training. The document additionally specified the project timeline and the arranged payment. However, 
Action Data did not have standardized documentation guidelines.
This was critical considering the fact that most of the workers worked remotely after the initial training at the company's office. %Upon project completion, the workers would receive an evaluation that included a quality score assigned by their supervisor and their payment. 
The only written records of how projects were conducted were emails between management and client, and Slack messages between data workers and management. %Moreover, Action Data's clients did not seem to be interested in having a better written record about the conduction of projects. Consequently, Action Data's management had, up until then, not seen the need for improving their documentation practices. 

%Company's founder Eva described her clients and their indifference towards documentation in the following interview excerpt:

%\begin{displayquote}
%I think that it's part because a lot of them are startups or individuals who do not have these business practices. But if you're working with a startup that just communicates by email very quickly and just sends over some of the images by email and just wants the JSON files with annotations back, they do they do not have the standard [documentation] practices.
%\end{displayquote}

%We interviewed a computer vision engineer working at one of Action Data's clients\,---\,a US-based company dedicated to producing contamination scanners driven by computer-vision technology. This client has turned to Action Data after being disappointed by the quality of annotations carried out through Amazon Mechanical Turk. The service Action Data provided for this client consisted of segmenting and labeling images of hands according to whether they present contamination or not. Like most of Action Data's client, this requester is a small tech company, which seems to have an effect on the client's disposition to document and the position documentation has in their priorities scale.  The informant described his company's position on documentation as follows:

%\begin{displayquote}
%So, the decisions about what's contamination and not isn't documented in words. It's documented in the images, I guess, is one way to think about it. And when I see a common thing that/ there are a few different characteristics about individuals’ hands in the environment that can actually look very much like contamination. And when I pick up on any one of those, I do send it out as a Slack message to the rest of engineering, being like, “Oh, this is something we might see,” to keep in mind. And then to the instructions that we give [Tina] and [Eva] at [Action Data], we've sent an email with instructions. I'll pull that up and send that along as well. [Documenting] is lower on our priority list than a bunch of other things that we need to do. It's just not the company's priority at this moment. There are other more valuable things to keep the company successful. As the engineering team grows, as we have more time to do those things and our work to meet the company's exact needs are less burdensome, then we'd go to more documentation 
%\end{displayquote}

After our first fieldwork period and once we had analyzed the collected data, we provided Action Data with a report summarizing our observations\,---\,most of them related to labor conditions, highlighting their effects on the quality of the datasets produced by the company.  In addition, we provided recommendations \textcolor{red}{regarding the need to educate data workers about the ML pipeline, the urgency of considering labor conditions an essential point in the “ethical AI” discourse at the core of the firm's marketing strategy, and the importance of documenting workflows and practices (REFERENCE ANONYMIZED)}. The company's management found that our suggestions were useful and actionable. By September 2020 they proceeded to implement some of them.

%\begin{displayquote}
%It was very enlightening to me that we have to invest more in our annotators’ understanding of the industry. And them understanding bias, understanding what their work is used for, why they're doing this type of annotation, what companies does it go for and so on. Because also that helps then improve their quality of work and their understanding of why one type of annotation is good or why one image collected is good versus another one[...] So, I think that us starting to develop training modules for bias in AI, understanding what AI is, what is our role in the whole ecosystem, that has been quite beneficial. And understanding the importance of keeping documentation! That was eye-opening! I think when you visited us, I wasn't doing that because I didn't have the bandwidth basically. 
%\end{displayquote}

It was around that time that we invited Action Data to participate in a series of follow-up interviews centered around documentation practices. The company had started developing an internal database of all the projects they had conducted since the beginning of their operations. %The database had properties like project name, status, who the client was, financial information such as invoices, pricing, advanced payment and incentive payment, project dates and description, names of the workers that worked on the project, and any written instructions provided to them. It also comprised feedback received from the clients after project completion. 
The implementation of this database was an important development. However, some of the information comprised in it was considered confidential or sensitive, what resulted in the documents only being shared with Action Data's management and the respective clients. The data workers did not have access to the project database. We provided feedback on this issue and highlighted the importance of sharing information with the data workers. The recently-hired operations officer, Tina, was then put in charge of creating a series of documents targeted to data workers, that contained guidelines and information about the different projects carried out by Action Data. Beyond our recommendation, two factors contributed to the company's decision to develop these documents. First, Action Data had managed to establish itself in the market of data services for machine learning\,---\,especially data labeling. This means that, by 2020, the company was conducting long-term projects for a more or less steady set of clients, which resulted in the need to keep better records and continually train workers. Second, because of its growth, the company had started outsourcing some requests to partner organizations located in Iraq and Syria. This development revealed the need for clear\,---\,written\,---\,guidelines for a geographically distributed workforce that, in most of the cases, did not speak English.

Since the inclusion of third-party organizations in the conduction of projects and because of the disadvantaged position of service providers vis-à-vis their clients, Action Data's perceived usefulness of documentation started to shift towards the idea of \emph{inter-organizational accountability}. The company started to develop a documentation template that was able to reflect its business relationship with other organizations, i.e. clients and partner organizations in the Middle East where projects were being increasingly outsourced. This form of documentation would make explicit each organization's responsibilities in terms of work, payment, and deadlines, and would reflect iterations and updates. Moreover, keeping clear records of the task instructions provided by clients and documenting instructed changes could provide proof that tasks were carried out as instructed, especially in cases where clients are not satisfied with the quality of the service provided or decide to demand more, as Eva explained:

\begin{displayquote}
We also keep the client accountable so that they don't come up with a new requirement or something that we haven't mentioned before. So, documents are also for accountability of us towards the client as well so that the client can have a document where they can keep track of what the arrangement is and so on beyond our contract.
\end{displayquote}

%This type of accountability would also become important when projects involved personal or sensitive data: 

%\begin{displayquote}
%They were trying to collect videos of people who are not moving and to compare them with still images. So, it was for the purposes of fraud detection so it was to distinguish when a person is showing an image versus their own face, even if the face is not moving. So, it was quite an interesting project and the company itself was a startup so we had to encourage them and wait for them to get everything sorted out in terms of GDPR and personal data protection, how the data would be stored and so on. And they also had to create, with our involvement, an agreement form before each person went on the platform to let's say donate their face[...] We had all the documentation and the terms and conditions of how the data would be used and so on.
%\end{displayquote}

Towards the beginning of 2021 and throughout several conversations and iterations, the idea of structuring documentation practices around three moments emerged: before starting the project, during the conduction of the project, and after the project is done. From then on, Action Data quickly began developing three documentation templates, each one aiming to reflect one of those three moments. The prototypes were designed as forms were information would be filled in by Action Data's management. When sending the prototypes to us to request feedback, operations manager Tina explained via email: 

\begin{displayquote}
On the first page is the \emph{SoW} (Scope of Work) that we regularly use in order to scope clients' projects before we start working. On the second one is a new idea Eva is piloting for \emph{Dataset Documentation}, so some information we will fill out during and after projects so that the client can use it for transparency purposes if they wish. And then the third page is a \emph{Post Mortem} template which we can use to address issues and challenges after the project is completed.
\end{displayquote}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.40]{BULGARIA_sow.png}
    \caption{One of the documentation templates prototyped by Action Data: The Scope of Work form (SoW).}
    \label{fig:sow}
\end{figure}

The \emph{SoW} form included information about the client, deadlines, preferred tools, acceptance and rejection standards, delivery format, annotation rules in the case of for data labeling tasks, and information about edge cases (see Fig. \ref{fig:sow}).  Upon our feedback, questions about the purpose and background of the project and about classes and labels for data collection and annotation were included.  The \emph{Dataset Documentation} form inquired about dataset size, taxonomy used for the annotation of the data, labeling team, labeling instructions, labeling methods, certainty score and edge cases. Upon our recommendation, a question about data provenance and collection method was added. The \emph{Post Mortem} template was developed to serve as a feedback form that management would fill out after project completion. It enquired about the conduction of projects and prompted reflection about goals, communication, timeline, workforce, quality, and lessons learned.
As we will describe in Section \ref{sec:FindWork}, these three prototypes were examined and interrogated at the co-design workshops that we run with Action Data workers.


\subsection{Summary and Look Forward}
\label{sec:FindSum}

Through the iterative process of \textit{conducting interviews -  providing feedback - observing as the organizations implemented ideas - and providing feedback again} some high-level findings became apparent: 
\begin{itemize}
    \item Data Documentation is collaborative.  Many actors take part in the documentation of data production processes. However, not every actor documenting or using documentation holds the same amount of power to shape documentation.
    \item Data Documentation should enable communication among actors and organizations and transport information that is useful and intelligible to all of them. 
    \item Data Documentation should not be seen as a one-time action. Data production projects requires living, evolving documents.
    \item Data Documentation should be part of current workflows and routines to foster a view of documentation as a constitutive part of data work.
    \item Data Documentation is context-based and should be adaptable to the specific needs of specific stakeholders.
\end{itemize}
We interpreted these findings as design considerations that we took into the co-design workshops along with the documentation prototypes developed by each company. 

Both BPOs were free in their interpretation of our observations and recommendations. In this sense, we perceived two different orientations in the way they implemented our feedback to create the documentation prototypes. While Alamo's documentation needs and ideas were oriented towards the \emph{preservation of knowledge} that could be useful to train (future) workers, Action Data had oriented its documentation efforts towards keeping \emph{inter-organizational accountability}, i.e., clearly stating clients' expectations and service providers’ responsibilities. %The two different orientations materialized in the documentation prototypes that we took into the respective workshops with each company: For the workshops with Alamo, the company proposed using the wiki-based documentation template that had been used to brief and train workers. Instead, Action Data proposed discussing the three templates that the company had recently prototyped, namely, the scope of work document, the dataset documentation, and the postmortem report. These prototypes were heavily oriented towards making explicit Action Data's relationships with its partners. 

These apparent differences were based on the corporate needs of each organization because, up until that point, the design process of the documentation prototypes had been piloted by the companies' founders and managers. However, at the co-design workshops, we learned that the needs of data workers at both organizations were not that different in terms of what they wanted to see reflected in documentation. As we will describe in the following section, the workshops would teach us that designing a documentation framework based on the needs and ideas of data workers would involve a different set of considerations.



\subsection{Lessons from the Workshops}
\label{sec:FindWork}

\subsubsection{Workshops with Alamo}
\label{sec:workshops-alamo}

The workshops with Alamo workers and managers started with a discussion of the documentation templates that the company had developed and recently implemented: the “kick-off” document describing the project and setting up the objectives, and a wiki-based website. 

The workshop’s first activity asked participants to reflect on these two templates. The discussion was carried out on the basis of a recent project from Alamo’s main client, the e-commerce corporation that operates primarily in Latin America. The client instructed Alamo to produce a training dataset with images of false identity cards from three Spanish-speaking Latin American countries. This dataset was later used for the client to train an algorithm to screen IDs. The instructions for workers involved the collection of images of authentic identification cards, their modification to render them invalid, and the labeling of the resulting photos. 

%Participants were organized in small groups of around five members in the second activity. Each group had to focus on a specific role in the data production process at Alamo: “analyst” (or data worker), “service owner” (team leaders), and “project manager.” Participants had to reflect on their involvement in each project phase for each role, which the company calls “kick-off,” “onboarding,” and project unfolding. We asked participants to reflect on the actions, interactions, reasoning, feelings, and documentation usage. We had formed these breakout groups based on participants' professional occupation because we wanted to avoid power dynamics interfering in the discussions and hoped to have a clear overview of the each group's needs. However, the discussions emerging from mixed groups and in plenum proved to be more constructive in allowing mutual learning.


%not sure if it fits here: this is perceived to be curious and at the same time insecure because of not knowing where it is going to take them/ what they will find: Bueno yo diría eso, como que están ahí curiosos y a la vez con este miedo de quiero saber, para donde nos va llevar o no saber con que lo que nos encontraremos. I: Se sienten inseguros digamos. B2: Inseguros. Como con ganas de hacer las cosas, pero bueno también eso como que lo tiene un poco- Pero bueno, es parte. (DIA1 ACT2A+3A - Transkript - TR217626, Pos. 44-46)

Led by the participants' interest, the discussions quickly centered on the Wiki as the first day of the workshop unfolded. By the end of day 1, it became evident that there is a discrepancy between how management thinks workers should use the Wikis and the latter’s perceived usefulness vis-à-vis the time and effort required to maintain it. As we mentioned earlier, one of Alamo’s main concerns as an impact source company is to foster skill development and learning opportunities among their workforce. Following this concern, managers participating at the workshop mentioned that the main benefit of the Wikis is for data workers to take an interest in existing projects, explore them through the respective Wikis, and use that information for their education and growth. In the words of a project manager:

\begin{displayquote}
We've been working with growth metrics for each person working at Alamo this year. For example, if someone wants to learn programming skills, they can look at the Wiki, see what tools are available, the projects, the languages used, and know what skills to develop.
\end{displayquote}

However, while managers want to encourage workers to have an overview of the undergoing projects at the company, they are also mindful of their clients’ demands in terms of confidentiality and security. For this reason, either much of the information in the documentation lacks details and appears general and superficial, or the access to such information is restrained. Several of the data workers reported that the restrictions and the lack of access to the Wikis as well as difficulties keeping the information updated represented a hurdle for their work:

\begin{displayquote}
One of the limitations is access that we all know the information is there and can access it. How can we make that happen? Not everyone has access. How can we guarantee that the information is updated? It takes much time to write down the documentation. 
\end{displayquote}

%In view of this claim, one of the project managers expressed being surprised because he had thought that most of the project descriptions and specifics were available to everyone:

%\begin{displayquote}
%I would have liked to hear about these issues from the workers directly. Because now that I think about it retrospectively, I honestly thought everyone had access because none of the data analysts ever told me ‘hey I can't see this or that’ or what they are saying now that they want to learn about the tools used in certain projects... nobody ever mentioned this to me! It is also a matter of being proactive.
%\end{displayquote}

During the discussion, some of the data workers asked the manages for trust in accessing complete versions of the documentation, but the managers argued that the information is sensitive and clients often request not to make it available to all. This tension, coupled with the difficulty of keeping documents updated as projects evolve, makes it hard for workers to incorporate feedback in the documentation due to the lack of information. 

Moreover, the workers acknowledged that they were less inclined to use the information on Wikis for references. For one thing, some workers were not aware that the Wikis were available for them to see other projects and had to be reminded of their presence. For another, the documentation was perceived as "on the machine" and "not close at hand" and, thus, it was not workers' initial responses to check if relevant information could be found on the Wikis.

We started the second workshop day with a focused discussion of the Wiki, specifically, the tensions identified during the previous session: how to keep the Wikis up to date, how to guarantee access and promote use, how to provide details while keeping confidentiality, and how to integrate documentation practices in existing workflows.
When discussing how to update the documentation efficiently, one of the data workers pointed out that gathering required information often took weeks due to the organizational structure and dispersed nature of teams.
In this discussion, possible ways for documentation were also explored. A former data analyst, now team leader, argued that automation was probably not the best solution because much information exchange and knowledge transfer took place in daily conversations, such in chats and emails. He regarded that opportunities of documentation lies in integrating documentation into communication processes: 

\begin{displayquote}
The record of what I do, the backup, an email, a chat […] because it happens to us that the approach in daily life leads you to solve without documenting or without recording or without warning. I think that's where the greatest possibility of improving communication lies. To leave at least a record. It does not necessarily have to be so precise to set up a whole process; but a spreadsheet where I document things, an e-mail, a chat. I don't know, there are many ways of communication. I don't know if the best thing is automation, because we are quite beyond automation. Yes, it is a matter of communication.
\end{displayquote}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.30]{ARGENTINA_co-design-activity.pdf}
    \caption{One of the activities conducted with Alamo's workers aiming at deconstructing and re-imagining documentation practices. The same activity was carried out with Action Data and one of its clients.}
    \label{fig:co-design}
\end{figure}

Finally, the last activity of day 2 asked workers to imagine possible approaches to the problems discussed earlier in the session. We divided participants into three breakout groups and asked them to think of a documentation process that would guarantee simplicity, accessibility, and integration in workflows. These requirements were derived from the previously-conducted interviews. The teams were invited to reflect on documentation format, components, information, actors, and actions. The composition of the groups was mixed and each team was comprised of managers and data workers.

In their own way, all teams focused on the use of documentation rather than the act of documenting. They all agreed that documentation should be easier to edit and interpret by any team member. In this sense, three themes were salient. First, the documents should have better navigation tools for readers. Some proposed additions include a history of editions (such as in other Wikis like Wikipedia) and a glossary to enable translation between languages and illustrate technology jargon. Second, documentation should be more legible. This improvement can be made by including visual material, such as graphics or video tutorials, and reducing text. Participants also proposed more interactive documentation. For example, teams can benefit from more precise structures instead of documents without format. Third, participants suggested three ways to increase participation in the documentation, i.e, by making everybody in the organization in charge of documenting, automating the passage between text input and the graphic output, and adding elements of gamification to encourage and measure participation. 

\subsubsection{Workshops with Action Data}

The workshops with Action Data’s workers, managers, and clients took place in three different sessions and followed a different structure as those with Alamo:
Day 1 (1.5 hours) gathered Action Data's management located in Bulgaria with 15 of its data workers (mostly data labelers) in Syria where Action Data outsources much of its business through a partner organization, the NGO Ranua.
Day 2 (3 hours) involved both Action Data's management and the workers in Syria. In addition, one of the BPO's client, namely, a group of three researchers from a Scandinavian university, took part in this session.
Day 3 (2 hours) was envisioned as a round table and only the Syrian data workers were invited to participate.
Communication among these globally distributed participants was enabled by simultaneous interpretations through audio channels in Arabic and English.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.30]{BULGARIA_ stakeholders.pdf}
    \caption{Stakeholder map showing the three groups participating in the second workshop session, the nature of their relationship, and the workflows that characterize it. The map was developed with the workshops participants.  The names of the organizations and individual actors, originally included in the stakeholder map, have been changed to be included in this paper}
    \label{fig:stakeholders}
\end{figure}

Day 1 focused on getting to know Action Data’s general structure and workflows, and discussing how stakeholders use the three documentation prototypes (“Scope of Work,” “Dataset Documentation,” “Postmortem Report”). To this end,  after a presentation section and a round of introductions, participants mapped the actions and relationships of each of the stakeholders in the data labeling process, from clients to Action Data’s intermediation, to their partners at Ranua, and workers in Syria (see Fig. \ref{fig:stakeholders}).  During this session, Action Data’s managers were observed to take an active, and even dominant, role in the discussion. Despite the facilitators' attempts to leave more space for data workers to share their perspectives, some of the managers kept on interrupting workers and taking over the conversation. This situation plus the deficient quality of some of the Arabic interpretations made communication extremely difficult and inhibited the data workers, resulting in most of them avoiding participation in the discussions and activities. 

In view of the faulty experience of day 1, we were forced to react quickly and change most of the concept we had designed for day 2 within 48 hours.  We first asked the Syrian workers for feedback and confirmed what the problem was. We then hired one more interpreter to support the Arabic channel and briefed all interpreters with key terms and vocabulary. In addition, we had one more Arabic-speaking facilitator joining the team, and prepared more breakout activities, arranging the teams according to language. Finally, several activities were adapted to highlight the focus on the experiences of data workers. With this new concept, we went into the second workshop day.

Day 2 started by recapping the stakeholders’ map created during the previous session (see Fig. \ref{fig:stakeholders}). The clients were then asked to place themselves in the map and explain the project they outsource with Action Data. The clients\,---\,three researchers at a Scandinavian university\,---\,were working on automating a safety system at the harbor front that would release a signal, for instance, if people fall in the water. The task that Action Data's workers performed for this client was related to the annotation of thermal videos from CCTV footage that would serve as training data. 

The first group activity of the day was a roleplay (see Fig. \ref{fig:roleplay}). We divided participants into three teams according to their role in the data production chain  (managers, requesters, data workers) and asked them to assume a different role: the clients roleplayed the data workers, the data workers assumed the role of the managers, and the managers roleplayed the requesters. We then asked each group to reflect on the knowledge required to conduct data-production projects in their assigned roles by filling information cards. Afterwards, each team presented they cards in a discussion round during which each group gave their feedback on how accurately it had been roleplayed by the others. For instance, the clients in the role of the data workers had generated many cards including questions about labeling type and classes, edge cases, desired output, and annotation precision. However, the feedback of the actual data workers surfaced two further issues that the clients who generate the questions had not contemplated. First, the data workers wanted to see a clear outline of the amount of their payment documented. And second, it was important to them to add a question about the possible ethical implications of the data they had to work with in terms of harms to data subjects as well as concerns about the mental health of data workers dealing with sensitive or triggering data. 

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.30]{BULGARIA_ roleplay_questions.pdf}
    \caption{Role play activity in breakout groups. Here the requester group had to generate questions (the yellow cards) assuming the role of the data labelers. Afterwards, the data labelers provided feedback and added their own questions (in the blue cards.)}
    \label{fig:roleplay}
\end{figure}

In the same discussion, workers considered the extent of annotation precision required an important information type because it defines the difficulty of the task and can have negative effects on the payment. This requirement is usually negotiated between requesters and managers, without the participation of data workers. %However, the data workers agreed that this fundamental issue should be negotiated between the requester and the Action Data's management because, in their view, the managers would have a better overview of what the data workers can afford: 
%\begin{displayquote}
%you know, the requester might say we want 100\%. But then the Humans in the Loop would be okay, like it's not, we can't do that. It's not humanly possible. We can do 90\%.
%\end{displayquote}

%The dispersion and intermediation\,---\,and power\,---\,of actors like Action Data and the Syrian organization Ranua also render pricing negotiation inaccessible to workers. These negotiations occur primarily between the client and Action Data with lesser participation of managers from Ranua, so the amount of intermediation leaves little room for workers to voice any concerns regarding payment. 
Following these discussions, participants acknowledged that one of the main problems of the documentation prototypes developed by Action Data is that they only involved managers and clients while ignoring data workers. Moreover, instruction documents for workers are translated into Arabic by Ranua’s management, placing a language barrier with the English-based documentation prototypes. 

Finally, the last activity of day 2 asked participants to imagine new forms of documentation by thinking of its format, structure, information, and the stakeholders involved in its development and access. 
Similarly to the Alamo team, Action Data's workers prioritized a view of documentation as a communication medium. Mostly, they acknowledged that documentation should allow the co-creation of task instructions with different stakeholders, particularly workers. In the words of one of the Syrian workers:

\begin{displayquote}
Communication and feedback should be the highest priorities. The biggest loser when communication is lacking is the annotators because they spend more effort and time adapting their work each time.
\end{displayquote}

In addition, by increasing the communication between different stakeholders, the documentation can potentially integrate feedback to make data-production processes clearer by reducing redundant work. Furthermore, it was discussed that a post-mortem report aiming at reflecting on the finished project allows producing knowledge for future projects. Such a document could include missing information, met goals, fairness in pricing and wages, the quality of the work environment, difficulties, and learned lessons. 

Day 3 was envisioned as a round table exclusively for data workers
%While planning the workshop sessions, we were aware of the issue of power dynamics and the influence of having managers and workers in the same session. 
and we hoped to enable a space for them to express their opinions and wishes without fear of professional repercussions.
%At the beginning of the session, we told the data workers about our decision of holding the meeting without the managers and asked for their opinion. They explicitly expressed their wish to hold the session as planed. 
%In fact, right at the beginning of the session, after mentioning feeling grateful for their job, several data workers expressed that there were certain conditions within their work that they would like to improve and agreed that they would feel uncomfortable discussing these issues in front of manages and clients. Throughout the session, they repeatedly thanked us for creating such an intimate space and for “hearing them out”.
Although all workshop sessions were designed to be about documentation practices, there were some more pressing needs that were the focus of the data workers, and that is to earn a living wage and be able to provide for their families. This way, we opened up the floor to discuss this issue and talk about possible approaches. After the workshops, we helped facilitate the dialogue \cite{bodker_bigissues_2018} between the Syrian data workers and Action Data management.  One of the main issues described by the workers was that they received the same payment regardless of their effort or time spent doing the tasks. One of the data workers explained the general feeling among her colleagues:

\begin{displayquote}
Some feel that the profit or the revenue they're making after the end of the job is not compared to the effort they have put into it. 
\end{displayquote}

Another issue with payment was the lack of room for negotiation by workers about their wages. For example, one practice that workers perceived as unfair was that management divided the client's payment equally among all team members regardless of individual efforts. Furthermore, the workers are not consulted in decisions about team composition and cannot influence how many workers will share the payment: 

\begin{displayquote}
When we divide the amount of money that we have received for that certain project, when it's divided by the number of people working on that project, so it turns out to be something completely unfair. 
\end{displayquote}

Tensions were observed during the discussion on the tools used to perform data work. The limitation of tools used by workers requires them to share accounts and keep a shared spreadsheet with the number of annotations per task that each worker had done. This  makes individual performances visible, accessible, and modifiable to all. One of the workshop participants explained that this was a practical choice due to the diverse working conditions and location of workers and the complexity in supervising and managing their work. He further emphasized mutual trust and confidence between the management and workers and among workers. \textcolor{red}{While acknowledging the honest behavior and mutual trust within teams, the others did not regard trust as a satisfying justification for the limitations of tools and pointed out that the problem was beyond trust issue. For one thing, current tools and arrangements posed difficulties in keeping track of and securing the tasks they individually performed. For another, they did not allow adequate respect for privacy, which could potentially undermine team solidarity. Therefore, other workers appealed for better tools and arrangements to facilitate work and} enhance privacy and security. In this sense, as a potential solution related to documentation efforts, the workers suggested that documentation should reflect how much workers are being paid and the purpose of their work. However, the individual earnings of each worker should remain private. %This improvement would serve as motivation for workers since the payment process could then become more transparent while still respecting the privacy of individuals.


\subsection{So What Do Data Workers Want to See Documented?}

The co-design workshops constituted a turning point in this investigation. Engaging in hands-on design sessions directly with data workers gave us the possibility to explore their needs and desiderata beyond corporate priorities. Moreover, the workshops gave us and the three participant groups, i.e., data workers, managers, and clients, the possibility to learn about their relationship, communication, and cooperation.

%The first design consideration to take into account involves establishing the roles of each stakeholder in the documentation process. These roles can vary according to the company, the client, and the project. There are, however, two patterns that can be derived from our findings.

%First, most of the information comes from the requesters and is documented by managers: The clients hold most of the relevant information and share it only with the BPO managers. The managers register that information in documents and act as gatekeepers, only granting access to the information according to the client's confidentiality-related requests.
%Second, data workers are expected to use the documentation: However, they receive only the bare minimum information that allows them to complete tasks according to client's instructions. Moreover, access is not always granted (as reported by Alamo's workers) and language translations can constitute a barrier (as discussed by Action Data's workers.)

%In sum, the information that out participants considered relevant and should be included in the documentation of data production projects is:
Here, we summarize and list some of our salient findings in terms of what data workers propose to include in documentation:
\begin{enumerate}
    \item \textbf{Who is the requester?}: Information about the client, its products, and its relationship history with the data processing company. 
    \item \textbf{What is the data going to be used for?}: Description of the ML product that will be trained on the basis of the data produced by data workers. The connection between the tasks performed by data workers and its use for the resulting ML model should be highlighted.
    \item \textbf{What kind of data are these?}: Including a warning in case of sensitive data.
    \item \textbf{Where do the data come from?}: Description of data provenance and dataset's previous uses. Proof of compliance with local regulations in the case of personal data. 
    \item \textbf{What should be done with the data?}: Description of task including categories and classes for annotation and collection.
    \item \textbf{How difficult is the task? How laborsome is this data?}:  Include a difficulty rating for workers to quickly estimate the workload and time required for the task.
    \item \textbf{What tools are used?}: Clear guidelines in terms of communication channels, software used to work on the data, and repository where the data will be stored.
    \item \textbf{Who is working on this project?}: Include information about team composition.
    \item \textbf{How much does this project pay to each data worker?}: Clear information about wages, payment structure, and rules.
    \item \textbf{How has the project and its documentation evolved over time?}: Include an updates history log, including date, time, and name of the person who documented each update.
    \item \textbf{What have we learned from this project?}: Include a post-mortem report to reflect upon edge cases, lessons learned, and possible mismatches between time, effort, and payment.
\end{enumerate}

\textcolor{red}{
%similarities
Workers at both sites wanted to have rigorous documentation on project requirements (items 5 and 7), ranging from what needs to be done and what not to what are the edge cases, acceptance and rejection standards, required quality, and format of end result etc. Information in this regard improves clarity of projects and offers a guideline for data work. They also wanted team composition (item 8) to be included to facilitate the coordination of team members and task division. Data workers in Action Data further required a special notification if the presence of specialists and experts was required.}


%differences
Workers at both sites wanted to have rigorous documentation on project requirements (items 5 and 7), ranging from what needs to be done and what not to what are the edge cases, acceptance and rejection standards, required quality, and format of end result etc. Information in this regard improves clarity of projects and offers a guideline for data work. They also wanted team composition (item 8) to be included to facilitate the coordination of team members and task division. Data workers in Action Data further required a special notification if the presence of specialists and experts was required.

The reasons motivating documentation practices can also vary.
Descriptions of data and projects (items 1-4) are desired to be documented for workers in Action Data, because they can help workers better understand projects and the requirements. Such improved understanding is especially helpful, when workers have to make discrete decisions in data work, or envision what the end result to be delivered might look like and orient their work towards it. For workers in Alamo, this information should be documented for the standardization purpose. Specifically on the involvement of sensitive data, a participant in Action Data wanted to know the potential use case of data and regarded this as a commitment from the clients that the data will not be used for inappropriate purposes. In comparison, workers in Alamo pointed to the need of clarification on how to process and store sensitive data to enhance confidentiality. 
Moreover, workers in Action Data attached value to the evaluation of project workload (item 6) and payment details (item 9), which could help them assess and decide the extent of commitment to the project, based on the perceived fairness of the pricing. In comparison, workers in Alamo placed more emphasis on the documentation on evolvement of projects (item 10). For one thing, given the regular communication within teams and between teams and clients, this can keep important decisions recorded and task instruction and requirements updated, which makes sure that workers are following the latest instructions. For another, metrics that measure performance at the individual and team levels serve as a basis for status check for projects and show if the team can accomplish tasks as planed, and if not, what are the coping strategies. 
Additionally, there is also divergence with respect to documentation of lessons learned from projects (item 11). While workers at both sites included a section to record things that went wrong and lessons learned in projects to inform and improve future projects at the team level, workers in Alamo also recognized that documentation in this regard could potentially be used to foster individual learning and growth.

==> Reserve/table.tex <==

\begin{tabular}{ c c  }
  Interviews & Workshop  \\
  Contradiction between company's mission of fostering worker growth and documentation practices oriented towards surveillance of workers through performance metrics & x \\
  Alamo's co-founder agreed to suggestions and expressed desire of establishing documentation practices based on needs of data workers & x
  
  7 & 8  \\
\end{tabular}

==> findingstable.tex <==
\begin{table}[ht]
\caption{Data Analysis: Summary of codes and themes}
\label{tab:codes}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.25\textwidth}p{0.3\textwidth}p{0.45\textwidth}}
\hline \hline
\multicolumn{1}{c}{\textbf{Domain Summaries}}          & \multicolumn{1}{c}{\textbf{Before the Workshop}} & \textbf{During/After the Workshop}                                                                                                                                    \\ \hline
\multirow{7}{0.25\textwidth}{FUNCTION OF DOCUMENTATION}             & Standardization                    & \multirow{13}{0.45\textwidth}{\textbf{DOCUMENTATION AS COMMUNICATION ENABLER ACROSS BOUNDARIES}}                                                                \\ \cline{2-2}
                                                       & Foster Workers Growth              &                                                                                                                                                    \\ \cline{2-2}
                                                       & Quality Control \& Metrics         &                                                                                                                                                    \\ \cline{2-2}
                                                       & Work Enabler                       &                                                                                                                                                    \\ \cline{2-2}
                                                       & Inter-org. Accountability &                                                                                                                                                    \\ \cline{2-2}
                                                       & Knowledge Peservation              &                                                                                                                                                    \\ \cline{2-2}
                                                       & Communication Medium               &                                                                                                                                                    \\ \cline{1-2}
\multirow{6}{0.25\textwidth}{ROLES AND COLLABORATION}               & Auditor                            &                                                                                                                                                    \\ \cline{2-2}
                                                       & Managers                           &                                                                                                                                                    \\ \cline{2-2}
                                                       & Service Owners                     &                                                                                                                                                    \\ \cline{2-2}
                                                       & Labelers                           &                                                                                                                                                    \\ \cline{2-2}
                                                       & BPO's Teams                        &                                                                                                                                                    \\ \cline{2-2}
                                                       & Clients                            &                                                                                                                                                    \\ \hline
\multirow{5}{0.25\textwidth}{DOCUMENTATION FORMATS}                 & Wiki                               & \multirow{10}{0.45\textwidth}{\textbf{HOW DOCUMENTATION CAN SUPPORT WORKERS’ AGENCY}}                                                                            \\ \cline{2-2}
                                                       & Kick-off Document                  &                                                                                                                                                    \\ \cline{2-2}
                                                       & Scope of Work (SoW)                &                                                                                                                                                    \\ \cline{2-2}
                                                       & Dataset Documentation              &                                                                                                                                                    \\ \cline{2-2}
                                                       & Postmortem Report                  &                                                                                                                                                    \\ \cline{1-2}
\multirow{5}{0.25\textwidth}{WORK ETHIC AND LABOR CONDITIONS}      & Impact and Responsibility          &                                                                                                                                                    \\ \cline{2-2}
                                                       & Trust                              &                                                                                                                                                    \\ \cline{2-2}
                                                       & Security                           &                                                                                                                                                    \\ \cline{2-2}
                                                       & Labor Conditions                   &                                                                                                                                                    \\ \cline{2-2}
                                                       & Confidenciality                    &                                                                                                                                                    \\ \hline
\multirow{6}{0.25\textwidth}{LIMITATIONS OF CURRENT DOC. PRACTICES} & Integration in Workflows           & \multirow{6}{0.45\textwidth}{\textbf{CHALLENGES DESIGNING FOR WORKERS IN CORPORATE ENVIRONMENTS}}                                                               \\ \cline{2-2}
                                                       & Use of Documentation               &                                                                                                                                                    \\ \cline{2-2}
                                                       & Lack of Information                &                                                                                                                                                    \\ \cline{2-2}
                                                       & Access                             &                                                                                                                                                    \\ \cline{2-2}
                                                       & Feedback                           &                                                                                                                                                    \\ \cline{2-2}
                                                       & Updates                            &                                                                                                                                                    \\ \hline
\multirow{8}{0.25\textwidth}{POSSIBLE DESIGN SOLUTIONS}             & Ownership                          & \multirow{8}{0.45\textwidth}{\textbf{DESIGN IDEAS EMERGED FROM THE WORKSHOPS}}                                                                                  \\ \cline{2-2}
                                                       & Synthesis /Simplicity              &                                                                                                                                                    \\ \cline{2-2}
                                                       & Interactivity                      &                                                                                                                                                    \\ \cline{2-2}
                                                       & Information Type                   &                                                                                                                                                    \\ \cline{2-2}
                                                       & Integration                        &                                                                                                                                                    \\ \cline{2-2}
                                                       & Centralizing                       &                                                                                                                                                    \\ \cline{2-2}
                                                       & Automation                         &                                                                                                                                                    \\ \cline{2-2}
                                                       & Visualization                      &                                                                                                                                                    \\ \hline
\multirow{4}{0.25\textwidth}{LESSONS}                             & Lessons from Fieldwork           & \multirow{4}{0.45\textwidth}{\textbf{WHAT PARTICIPANTS \& ORGANIZERS LEARNED THROUGH THE CO-DESIGN PROCESS}} \\ \cline{2-2}
                                                       & Lessons from our Feedback        &                                                                                                                                                    \\ \cline{2-2}
                                                       & Lessons from the Interviews      &                                                                                                                                                    \\ \cline{2-2}
                                                       & Lessons from he Workshops       &                                                                                                                                                    \\ \hline \hline
\end{tabular}
}
\end{table}

\begin{table}[]
\caption{\textcolor{red}{Overview of Participants and Research Methods. Some participants were interviewed more than once.}}
\label{tab:participants}
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.08\textwidth}p{0.14\textwidth}p{0.27\textwidth}p{0.2\textwidth}p{0.14\textwidth}p{0.17\textwidth}} \hline \hline \small
\textbf{Method} & \multicolumn{1}{c}{\textbf{Organization}} & \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\textbf{Participants}} & \multicolumn{1}{c}{\textbf{Medium}} & \multicolumn{1}{c}{\textbf{Language}} \\ \hline 
\multirow{7}[23]{*}{{\rotatebox[origin=c]{90}{\small \textbf{SEMI-STRUCTURED INTERVIEWS}}}} & Alamo & BPO in Argentina & 6 data workers & In-Person & Spanish \\
 & Alamo & BPO in Argentina & 2 managers & In-Person & Spanish \\ \cline{2-6}
 & Action Data & BPO in Bulgaria & 9 data workers & In-Person & English with Arabic interpretation \\
 & Action Data & BPO in Bulgaria & 2 managers & In-Person & English \\  \cline{2-6}
 & Alamo's clients & ML Practitioners requesting data work from Alamo & 1 requesters & Virtual & Spanish \\  \cline{2-6}
 & Action Data's clients & ML Practitioners   requesting data work from Action Data & 5 requesters & Virtual & English \\  \cline{2-6}
 & Other Clients & ML Practitioners requesting data   work from other BPOs & 4 requesters & Virtual & English \\ \hline 
\multirow{7}[17]{*}{{\rotatebox[origin=c]{90}{\small \textbf{CO-DESIGN WORKSHOPS}}}} & Action Data & BPO in Bulgaria & 2 managers & \multirow{5}{*}{Virtual} & \multirow{5}{0.17\textwidth}{English with Arabic interpretation} \\
 & Action Data & BPO in Bulgaria & 2 data workers &  &  \\  \cline{2-4}
 & Ranua & Action Data's Syrian partner organization & 1 manager &  &  \\
 & Ranua & Action Data's Syrian partner organization & 13 data workers &  &  \\ \  \cline{2-4}
 & Action Data's clients & ML Engineers at Scandinavian University & 3 requesters &  &  \\  \cline{2-6}
 & Alamo & BPO in Argentina & 13 data workers & \multirow{2}{*}{Virtual} & \multirow{2}{*}{Spanish} \\
 & Alamo & BPO in Argentina & 4 managers &  & \\ \hline \hline 
\end{tabular}
}
\end{table}
